Mechanical design and fabrication of a kinetic sculpture with application to bioinspired drone design

Biologically-inspired robots are a very interesting and difficult branch of robotics dues to its very rich dynamical and morphological complexities. Among them, flying animals, such as bats, have been among the most difficult to take inspiration from as they exhibit complex wing articulation. We attempt to capture several of the key degrees-of-freedom that are present in the natural flapping gait of a bat. In this work, we present the mechanical design and analysis of our flapping wing robot, the Aerobat, where we capture the plunging and flexion-extension in the bat's flapping modes. This robot utilizes gears, cranks, and four-bar linkage mechanisms to actuate the arm-wing structure composed of rigid and flexible components monolithically fabricated using PolyJet 3D printing. The resulting robot exhibits wing expansion and retraction during the downstroke and upstroke respectively which minimizes the negative lift and results in a more efficient flapping gait.

==> unused.tex <==
\subsubsection{Humerus Mechanism Optimization}

The humerus mechanism is optimized using the cost function $\bm{y} = \bm{\hat{\theta}}_s - \bm{\theta}_s$ where $\bm{\theta}_s$ is the trajectory vector gained by solving \eqref{eq:kin_constraint} for $\theta_{s,k}$ given the input angle $\theta_{1,k} = 2\pi k/N + \phi_0$, $k = \{1,\dots,N\}$. We then optimize the following 13 parameters
%
\begin{equation}
\begin{aligned}
\bm{q}_{H} = [ &l_{1}, l_{2}, l_{3a}, l_{3b}, l_{3c}, l_{4}, l_{5a}, l_{5b}, \\
&\alpha_5, p_{4y}, p_{7x}, p_{7y}, \phi_0] ,
\end{aligned}
\end{equation}
%
subject to the following constraints: (1) the body-fixed joint positions ($\bm{p}_4$ and $\bm{p}_7$) are within the the robot's 50 mm diameter cylindrical body, (2) the linkages don't intersect or block each other, and (3) the length constraints for the linkages to prevent singularity in the four-bar mechanism. For example, the constraint equation $(l_1 + |\bm{p}_4 - \bm{p}_1|) - 0.8\,(l_2 + l_{3a}) < 0$ constrains the linkage lengths to prevent singularity in the four-bar mechanism ($J_{1}$, $J_{2}$, $J_{3}$, $J_{4}$). We use a similar constraint for the other four-bar mechanisms.


\subsubsection{Radius Mechanism Optimization}

Once the humerus parameters has been optimized, we can then optimize the remaining 17 parameters for the radius mechanism
%
\begin{equation}
\begin{aligned}
\bm{q}_{R} = [ &l_{6}, l_{7}, l_{8a}, l_{8b}, l_{8c}, l_{9}, l_{10a}, l_{10b}, l_{10c}, \\ &l_{10d}, l_{11}, l_{12a}, l_{12b}, p_{12y}, p_{14x}, p_{14y}, \Delta \phi] ,
\end{aligned}
\end{equation}
%
subject to similar constraints and follow the same procedures as the humerus optimization problem. The cost function calculates the trajectory error $\bm{y} = \bm{\hat{\theta}}_e - \bm{\theta}_e$.
